On the welded Tube map

This note investigates the so-called Tube map which connects welded knots, that is a quotient of the virtual knot theory, to ribbon torus-knots, that is a restricted notion of fillable knotted tori in the 4-sphere. It emphasizes the fact that ribbon torus-knots with a given filling are in one-to-one correspondence with welded knots before quotient under classical Reidemeister moves and reformulates these moves and the known sources of non-injectivity of the Tube map in terms of filling changes.

==> MySetting.tex <==
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage{amsfonts,amsthm,amssymb,amsmath,latexsym,wasysym,stmaryrd,mathrsfs}
\usepackage{multirow,rotating,subfigure,picins,graphicx,bigstrut,lscape}
\usepackage{hyperref}
\usepackage{appendix}
\usepackage{makeidx}
\usepackage[centerlast]{caption}

\usepackage{fancyhdr}

\usepackage{pdftricks}
\usepackage{color}
\usepackage[all,color]{xy}


\graphicspath{{Figures/}}


\setlength{\oddsidemargin}{10pt}
\setlength{\evensidemargin}{10pt}
\addtolength{\topmargin}{-30pt}
\setlength{\textwidth}{430pt}
\setlength{\textheight}{640pt}
\setlength{\headheight}{15pt}
\setlength{\headsep}{30pt}
\setlength{\captionmargin}{1cm}


\newtheorem {theo}{Theorem}[section]
\newtheorem {theo*}{Theorem}[]
\newtheorem {lemme}[theo]{Lemma}
\newtheorem {lemme*}[theo*]{Lemma}
\newtheorem {prop}[theo]{Proposition}
\newtheorem {prop*}[theo*]{Proposition}
\newtheorem {cor}[theo]{Corollary}
\newtheorem {cor_proof}[theo]{Corollary (of the proof)}
\newtheorem {cor*}[theo*]{Corollary}
\newtheorem {cor_proof*}[theo*]{Corollary (of the proof)}
\newtheorem {conjecture}{Conjecture}[]
\theoremstyle{definition}
\newtheorem {defi}[theo]{Definition}
\newtheorem {defi*}[theo*]{Definition}
\newtheorem {nota}[theo]{Notation}
\newtheorem {nota*}[theo*]{Notation}
\newtheorem {question}[theo]{Question}
\newtheorem {question*}[theo*]{Question}
\theoremstyle{remark}
\newtheorem {remarque}[theo]{Remark}
\newtheorem {remarque*}[theo*]{Remark}
\newtheorem {exemple}[theo]{Example}
\newtheorem {exemple*}[theo*]{Example}
\newtheorem {fact}[theo]{Fact}
\newtheorem {fact*}[theo*]{Fact}


\def\e{\varepsilon}
\def\h{\mathfrak{h}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\F{{\mathcal F}}
\def\FF{{\mathbb F}}
\def\H{\mathfrak{H}}
\def\HH{\mathcal{H}}
\def\I{{\mathcal I}}
\def\II{{\mathscr I}}
\def\J{{\mathcal J}}
\def\K{{\mathcal K}}
\def\L{{\mathcal L}}
\def\M{{\mathcal M}}
\def\N{{\mathbb N}}
\def\O{{\mathbb O}}
\def\P{\mathfrak{P}}
\def\R{{\mathbb R}}
\def\S{{\mathbb S}}
\def\SS{{\mathfrak S}}
\def\T{{\mathcal T}}
\def\X{{\mathbb X}}
\def\Z{{\mathbb Z}}
\def\2Z{{\fract{\Z}/{2\Z}}}

\def\p{\partial}
\def\Sn{{\widetilde{\SS}_n}}


\def\Cone{{\textnormal{Cone}}}
\def\Hom{{\textnormal{Hom}}}
\def\Id{{\textnormal{Id}}}
\def\Im{{\textnormal{Im}}}
\def\Int{{\textnormal{Int}}}
\def\Ker{{\textnormal{Ker}}}
\def\Sei{{\textnormal{Sei}}}

\def\deg{{\textnormal{deg}}}
\def\gr{{gr}}
\def\ie{{\it i.e. }}
\def\qdim{{\textnormal{{\it q}-dim}}}
\def\rk{{\textnormal{rk}}}

%\def\siecle#1{\textsc{\romannumeral #1}\textsuperscript{e}~siècle}


\newcommand{\noi}{\noindent}
\newcommand{\disp}{\displaystyle}
\newcommand{\saut}{\vspace{\baselineskip}}

\def\fract#1/#2{\hbox{\leavevmode
  \kern.1em \raise .25ex \hbox{\the\scriptfont0 $#1$}\kern-.1em }\big/
  {\hbox{\kern-.15em \lower .5ex \hbox{\the\scriptfont0 $#2$}} }}

\newcommand{\dessin}[2]{
  \vcenter{\hbox{\includegraphics[height=#1]{#2.pdf}}}}
\newcommand{\dessinH}[2]{
  \vcenter{\hbox{\includegraphics[width=#1]{#2.pdf}}}}

\newcommand{\func}[3]{
  #1 \colon #2 \longrightarrow #3}
\newcommand{\plong}[3]{
  #1 \colon #2 \hookrightarrow #3}
\newcommand{\function}[5]{
  #1 \colon
  \begin{array}{ccc}
    #2 & \longrightarrow & #4\\[.2cm]
    #3 & \longmapsto & #5
  \end{array}}

%\makeindex
